Shape-Constraint Recurrent Flow for 6D Object Pose Estimation

Most recent 6D object pose methods use 2D optical flow to refine their results. However, the general optical flow methods typically do not consider the target's 3D shape information during matching, making them less effective in 6D object pose estimation. In this work, we propose a shape-constraint recurrent matching framework for 6D object pose estimation. We first compute a pose-induced flow based on the displacement of 2D reprojection between the initial pose and the currently estimated pose, which embeds the target's 3D shape implicitly. Then we use this pose-induced flow to construct the correlation map for the following matching iterations, which reduces the matching space significantly and is much easier to learn. Furthermore, we use networks to learn the object pose based on the current estimated flow, which facilitates the computation of the pose-induced flow for the next iteration and yields an end-to-end system for object pose. Finally, we optimize the optical flow and object pose simultaneously in a recurrent manner. We evaluate our method on three challenging 6D object pose datasets and show that it outperforms the state of the art significantly in both accuracy and efficiency.

==> defs.tex <==
% !TEX root = top.tex
% !TEX spellcheck = en-US

\newif\ifdraft
\draftfalse
\drafttrue

\usepackage{xcolor}
\definecolor{orange}{rgb}{1,0.5,0}
\definecolor{violet}{RGB}{70,0,170}

\ifdraft
 \newcommand{\YH}[1]{{\color{blue}{\bf YH: #1}}}
 \newcommand{\yh}[1]{{\color{blue}{#1}}}
 \newcommand{\Yang}[1]{{\color{violet}{\bf Yang: #1}}}
 \newcommand{\yang}[1]{{\color{violet}{#1}}}
\else
 \newcommand{\YH}[1]{}
 \newcommand{\yh}[1]{{#1}}
 \newcommand{\Yang}[1]{}
\fi

% \newcommand{\comment}[1]{}
\newcommand{\parag}[1]{\vspace{-3mm}\paragraph{#1}}

% Matrices
\newcommand{\bA}{\mathbf{A}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bR}{\mathbf{R}}
\newcommand{\btA}{\tilde{\mathbf{A}}}
\newcommand{\bbA}{\bar{\mathbf{A}}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bXe}{\tilde{\mathbf{X}}}
\newcommand{\bbX}{\bar{\mathbf{X}}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bte}{\tilde{\mathbf{e}}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\bp}{\mathbf{p}}
\newcommand{\bt}{\mathbf{t}}

\def\bSigma{\boldsymbol\Sigma}

\newcommand{\minimize}{\operatornamewithlimits{minimize}}


==> figure/framework_compare.tex <==
\begin{tabular}{c}
   \includegraphics[width=0.9\linewidth]{figure/arch_compare/framework_compare_flow.pdf} \\
   (a) The typical shape-unaware framework.\\[5pt]
   \includegraphics[width=0.9\linewidth]{figure/arch_compare/idea_middle.pdf} \\
   (b) The typical shape-unaware framework.\\[5pt]
   \includegraphics[width=0.9\linewidth]{figure/arch_compare/framework_compare_ours.pdf} \\
   (c) Our shape-aware framework.\\
\end{tabular}



==> figure/motivation.tex <==
% \begin{figure}
%     \setlength\tabcolsep{2pt}
%     \begin{tabular}{cccc}
%        \includegraphics[scale=0.21]{figure/motivation/ref_pose.png} & 
%        \setlength{\fboxsep}{0.5pt}\setlength{\fboxrule}{0.25pt}\fbox{\includegraphics[scale=0.21]{figure/motivation/flow_flow.png}} & 
%        \includegraphics[scale=0.21]{figure/motivation/flow_fw.png} & 
%        \includegraphics[scale=0.21]{figure/motivation/flow_res.png} \\
%        \includegraphics[scale=0.21]{figure/motivation/ref_render.png}&
%        \setlength{\fboxsep}{0.5pt}\setlength{\fboxrule}{0.25pt}\fbox{\includegraphics[scale=0.21]{figure/motivation/pose_flow.png}} & 
%        \includegraphics[scale=0.21]{figure/motivation/pose_fw.png} & 
%        \includegraphics[scale=0.21]{figure/motivation/pose_res.png} \\
%        \makecell{Reference\\Pose} &\makecell{Estimated\\Flow} &\makecell{Forward\\Warp} & \makecell{Refinement}
%     \end{tabular}
%     \caption{
%     \textbf{Top row:} Given a reference pose, one can use a typical optical flow estimation network to estimate the 2D-2D correspondences between the rendered image and the target image.
%     However, the forward warp result shows that the estimated flow can not preserve shape well.
%     \textbf{Bottom row:} In our pose-driven framework, the flow rendered by relative pose can naturally preserve shape because of the property of rigid transformation.
%     Using the shape-aware flow to index correlation, we can introduce the geometry bias, benefiting the pose regression.
%     Thus, we can produce a much better pose than shape-unaware flow.
%     }
%     \label{fig:motivation}
%  \end{figure}
% \begin{figure}
%    \centering
%    \setlength{\abovecaptionskip}{0.cm}
%    \includegraphics[width=0.95\linewidth]{figure/motivation/motivation.pdf}
%    \caption{
%    \textbf{Top row:} In the iterative flow estimation framework, we update the current state by the estimated 2D-2D correspondences.
%    As can be seen, the transformed state can not preserve shape.
%    Comparing the target image with such a sequence of 2D-shape-unaware states can not provide a clue about the 3D shape.
%    \textbf{Bottom row:} In our pose-driven framework, we project the 3D shape by the estimated pose, yielding a shape-preserve state.
%    Comparing the target image with the perspective 3D shape's multi-view projections helps to clarify the 3D shape.
%    Introducing such a 3D shape prior knowledge will benefit the pose regression.
%    }
%    \label{fig:motivation}

% \end{figure}

% \begin{figure}[t]
%   \centering
%   \begin{tabular}{c}
%       \includegraphics[width=0.9\linewidth]{figure/motivation/2D-3D corr.pdf} \\
%       \small{(a) Basic structure based on 2D-3D correspondence}\\[10pt]
%       \includegraphics[width=0.9\linewidth]{figure/motivation/2D-2D corr.pdf} \\
%       \small{(b) Basic structure based on 2D-2D correspondence} \\[10pt]
%       \includegraphics[width=0.9\linewidth]{figure/motivation/shape-aware 2D-2D corr.pdf} \\
%       \small{(c) Basic strcture of our method} \\
%   \end{tabular}
%   \caption{
%       \textbf{Comparison of different 6D pose estimation paradigms.}
%   }
%   \label{fig:motivation}
% \end{figure}
 
 
% \begin{tabular}{ccc}
%     \includegraphics[width=0.4\linewidth]{figure/visualization/000048_001212_real.png}&
%     \includegraphics[width=0.4\linewidth]{figure/visualization/000048_001212_render.png} \\
%     {\small (a) Target Image}    & {\small (b) Reference Image} \\
%     \includegraphics[width=0.4\linewidth]{figure/visualization/flow/000048_001212_iter1_fw.png} & 
%     \includegraphics[width=0.4\linewidth]{figure/visualization/pose/000048_001212_iter1_fw.png} \\
%     \makecell[c]{\small{(c) Shape-unaware} \\\small{Correspondence}}    & \makecell[c]{{\small (d) Shape-informed} \\ {\small Correspondence}} \\
%     % \includegraphics[width=0.4\linewidth]{figure/visualization/flow/000048_001212_iter2_fw.png} &
%     % \includegraphics[width=0.4\linewidth]{figure/visualization/pose/000048_001212_iter2_fw.png} \\
%     \includegraphics[width=0.4\linewidth]{figure/visualization/flow/000048_001212_res.png} &
%     \includegraphics[width=0.4\linewidth]{figure/visualization/pose/000048_001212_res.png} \\
%     {\small (e) baseline pose results}       & {\small (f) Our pose results}\\
% \end{tabular}

\begin{tabular}{c@{\hspace{3em}}c}
    \includegraphics[width=0.45\linewidth]{figure/motivation/architecture_flow.pdf} &
    \includegraphics[width=0.45\linewidth]{figure/motivation/architecture_ours.pdf} \\
    \small{(a) The standard strategy} & \small{(b) Our strategy} \\
\end{tabular}
% \begin{tabular}{c|cc}
%     \includegraphics[width=0.33\linewidth]{figure/visualization/000048_001212_render.png} & 
%     \includegraphics[width=0.33\linewidth]{figure/visualization/flow/000048_001212_iter1_fw.png} & 
%     \includegraphics[width=0.33\linewidth]{figure/visualization/flow/000048_001212_res.png} \\
%     {\small (a) Reference Image}   & \multicolumn{2}{c}{\small{(c) Shape-unaware Correspondence}} \\
%     \includegraphics[width=0.33\linewidth]{figure/visualization/000048_001212_real.png}&
%     \includegraphics[width=0.33\linewidth]{figure/visualization/pose/000048_001212_iter1_fw.png} &
%     \includegraphics[width=0.33\linewidth]{figure/visualization/pose/000048_001212_res.png} \\
%     {\small (b) Target Image} & \multicolumn{2}{c}{{\small(d) Shape-informed Correspondence}}\\
%     % {\small (a) Target Image}    & {\small (b) Reference Image} \\
%     % \includegraphics[width=0.4\linewidth]{figure/visualization/flow/000048_001212_iter1_fw.png} & 
%     % \includegraphics[width=0.4\linewidth]{figure/visualization/pose/000048_001212_iter1_fw.png} \\
%     % \makecell[c]{\small{(c) Shape-unaware} \\\small{Correspondence}}    & \makecell[c]{{\small (d) Shape-informed} \\ {\small Correspondence}} \\
%     % % \includegraphics[width=0.4\linewidth]{figure/visualization/flow/000048_001212_iter2_fw.png} &
%     % % \includegraphics[width=0.4\linewidth]{figure/visualization/pose/000048_001212_iter2_fw.png} \\
%     % \includegraphics[width=0.4\linewidth]{figure/visualization/flow/000048_001212_res.png} &
%     % \includegraphics[width=0.4\linewidth]{figure/visualization/pose/000048_001212_res.png} \\
%     % {\small (e) baseline pose results}       & {\small (f) Our pose results}\\
% \end{tabular}
% \begin{tabular}{ccccc}
%     \includegraphics[width=0.2\linewidth]{figure/visualization/000050_001189/render.png} & 
%     \includegraphics[width=0.2\linewidth]{figure/visualization/000050_001189/render.png} & 
%     \includegraphics[width=0.2\linewidth]{figure/visualization/000050_001189/flow_flow.png} & 
%     \includegraphics[width=0.2\linewidth]{figure/visualization/000050_001189/flow_corr.png} & 
%     \includegraphics[width=0.2\linewidth]{figure/visualization/000050_001189/real.png} \\
%     (a) 3D Shape & (b) Reference & (c) Dense Flow  & (d) Shape-unaware      & (e) Target
% \end{tabular}

==> figure/vis_response_map.tex <==
\begin{figure}[h]
    \centering
    \setlength\tabcolsep{1pt}
    \begin{tabular}{cccc}
       \includegraphics[width=0.24\linewidth]{figure/vis_response_map/000058_000030_real.png} & 
       \includegraphics[width=0.24\linewidth]{figure/vis_response_map/000058_000030_render.png} &
       \includegraphics[width=0.24\linewidth]{figure/vis_response_map/000058_000030_flow.png} &
       \includegraphics[width=0.24\linewidth]{figure/vis_response_map/000058_000030_pose.png} \\
       \includegraphics[width=0.24\linewidth]{figure/vis_response_map/000049_000001_real.png} & 
       \includegraphics[width=0.24\linewidth]{figure/vis_response_map/000049_00001_render.png} &
       \includegraphics[width=0.24\linewidth]{figure/vis_response_map/000049_000001_flow.png} &
       \includegraphics[width=0.24\linewidth]{figure/vis_response_map/000049_000001_pose.png} \\
       \includegraphics[width=0.24\linewidth]{figure/vis_response_map/000058_000001_real.png} & 
       \includegraphics[width=0.24\linewidth]{figure/vis_response_map/000058_000001_render.png} & 
       \includegraphics[width=0.24\linewidth]{figure/vis_response_map/000058_000001_flow.png} &
       \includegraphics[width=0.24\linewidth]{figure/vis_response_map/000058_000001_pose.png} \\
       \includegraphics[width=0.24\linewidth]{figure/vis_response_map/000052_000164_real.png} & 
       \includegraphics[width=0.24\linewidth]{figure/vis_response_map/000052_000164_render.png} & 
       \includegraphics[width=0.24\linewidth]{figure/vis_response_map/000052_000164_flow.png} &
       \includegraphics[width=0.24\linewidth]{figure/vis_response_map/000052_000164_pose.png} \\
 
       (a) & (b) & Baseline & Ours\\
    \end{tabular}
    \caption{
       \textbf{Response map between the target image and a query point in the reference image.}
       Query point in reference patch is visualized by the green square, and its corresponding point is visualized in the target patch.
       For the distinguishable query point(top and second row), our method can provide much less spurious correlations and much 
       At the third and last row, the query points are texture-less, making them indistinguishable.
       Nevertheless, our method success to respond to the query point, while the baseline fails to provide right correlations.
    }
    \label{fig:response_map}
 \end{figure}
